SDRS: Shape-Differentiable Robot Simulator

Robot simulators are indispensable tools across many fields, and recent research has significantly improved their functionality by incorporating additional gradient information. However, existing differentiable robot simulators suffer from non-differentiable singularities, when robots undergo substantial shape changes. To address this, we present the Shape-Differentiable Robot Simulator (SDRS), designed to be differentiable under significant robot shape changes. The core innovation of SDRS lies in its representation of robot shapes using a set of convex polyhedrons. This approach allows us to generalize smooth, penalty-based contact mechanics for interactions between any pair of convex polyhedrons. Using the separating hyperplane theorem, SDRS introduces a separating plane for each pair of contacting convex polyhedrons. This separating plane functions as a zero-mass auxiliary entity, with its state determined by the principle of least action. This setup ensures global differentiability, even as robot shapes undergo significant geometric and topological changes. To demonstrate the practical value of SDRS, we provide examples of robot co-design scenarios, where both robot shapes and control movements are optimized simultaneously.

==> figures.tex <==
\iffalse 
\begin{figure*}[ht]
\centering
\scalebox{.75}{
\begin{tabular}{cc}
\includegraphics[width=.4\textwidth]{figs/snake/snake.pdf} &
\includegraphics[width=.43\textwidth]{figs/snake/sum_snake.pdf}
\end{tabular}}
%\vspace{-10px}
\caption{\label{fig:snake}Compared with the original snake's foot shape (left), our optimized foot (middle) has a flat contact surface as highlighted, which improves friction and thus leads to better locomotion performance (right).}
\end{figure*}
\fi

\iffalse 
\begin{figure*}[ht]
\centering
\begin{tabular}{cc}
\includegraphics[width=.55\textwidth]{figs/spider/foot.pdf}&
\includegraphics[width=.34\textwidth]{figs/spider/sum_spider.pdf}
\end{tabular}
%\vspace{-10px}
\caption{\label{fig:spider}Similarly to the case with the snake, our co-optimization leads to a larger improvement in our spider's example. From left to right, we show the original leg shape, optimized leg shape, and the convergence history.}
\end{figure*}
\fi

\iffalse 
\begin{figure*}[ht]
\centering
\setlength{\tabcolsep}{1px}
\begin{tabular}{cccc}
\includegraphics[trim=4cm 0 4cm 0,clip,height=.25\textwidth]{figs/hole/hole_fig/first0.png}&
\includegraphics[trim=4cm 0 4cm 0,clip,height=.25\textwidth]{figs/hole/hole_fig/final0.png}&
\includegraphics[trim=4cm 0 4cm 0,clip,height=.25\textwidth]{figs/hole/hole_fig/final1.png}&
\includegraphics[height=.25\textwidth]{figs/hole/hole.pdf}
\end{tabular}
%\vspace{-10px}
\caption{\label{fig:hole}We use co-design to carve a hole in the red block to have the yellow peg settle at a $45.8^\circ$-tilted pose on it. From left to right: The initial configuration of the two bodies; the optimized red block with the hole carved; the simulated settling pose of the peg; and the convergence history of the benchmark.}
\end{figure*}
\fi
